FUSEE: A Fully Memory-Disaggregated Key-Value Store (Extended Version)

Distributed in-memory key-value (KV) stores are embracing the disaggregated memory (DM) architecture for higher resource utilization. However, existing KV stores on DM employ a semi-disaggregated design that stores KV pairs on DM but manages metadata with monolithic metadata servers, hence still suffering from low resource efficiency on metadata servers. To address this issue, this paper proposes FUSEE, a FUlly memory-diSaggrEgated KV StorE that brings disaggregation to metadata management. FUSEE replicates metadata, i.e., the index and memory management information, on memory nodes, manages them directly on the client side, and handles complex failures under the DM architecture. To scalably replicate the index on clients, FUSEE proposes a client-centric replication protocol that allows clients to concurrently access and modify the replicated index. To efficiently manage disaggregated memory, FUSEE adopts a two-level memory management scheme that splits the memory management duty among clients and memory nodes. Finally, to handle the metadata corruption under client failures, FUSEE leverages an embedded operation log scheme to repair metadata with low log maintenance overhead. We evaluate FUSEE with both micro and YCSB hybrid benchmarks. The experimental results show that FUSEE outperforms the state-of-the-art KV stores on DM by up to 4.5 times with less resource consumption.

==> QuestionList.tex <==
P1: Please provide more details about your experimental setup, to help the reviewers interpret the results. For example, do all results (microbenchmark and YCSB) use only a single index replica and two data replicas, and if so, how does FUSES' SNAPSHOT replication protocol work?

P2: The YCSB evaluation data set (100k keys of 1024-byte values) is quite small; how well does FUSES work for larger datasets and for datasets with smaller values?

M1: What problem does FUSES solve? 

D1: What are the pros and cons of maintaining separate metadata servers vs. storing metadata with the data (e.g., scalability, fault tolerance)? Is a fully memory-disaggregated KVS design the only approach for addressing the problem you target?

D2: What are the requirements for FUSES' memory management, and what can be handled by the client vs. what must be handled by the memory node (MN)? How well would a MN-only solution perform?

D3: Please clarify how the proposed 2-level memory allocation/free is used in the context of read and write operations. For example, how does FUSES reclaim the memory space of old KV pairs?

% More questions
How does FUSES compare with Dinomo? (RB)

(Adaptive Cache Issue) For example, as shown in Figure 10c, is the search latency of FUSES without this optimization worse than that of Clover? (RE)

How many of your design decisions were in reaction to this earlier architecture vs. choices that you would have proactively made if you were designing FUSES from scratch? (RB)

How are the primary and backup replica locations (e.g., MMI, Index, KV pairs) chosen? Are they coordinated, to avoid hot spots from placing too many primaries on the same node? (RB)

How do you ensure that the master is fault tolerant? (RB)

For SEARCH where CLOVER seems to have lower latency? (RC)

(Evaluation of Resource Utilization) In the introduction, it was discussed that FUSES can achieve full resource utilization. However, it seems that the resource utilization of FUSES, compared to the previous approaches, is not discussed in the evaluation. (RD)

How would the presence of additional DM computational capabilities impact FUSES' design? (RB)

How does the FUSES architecture generalize beyond a key-value store to a broader set of applications (e.g., graph store, machine learning parameter server, file system)?

Term: partially disaggregated, holistic memory management, primary memory region

% 没回答的
For the embedded operation log scheme, its overhead can be analyzed and compared with existing techniques. (RD)

Your notion of two-level memory management is reminiscent of what HP did in The Machine. See Paolo Faraboschi, et al., "Beyond processor-centric operating systems," Proc. HotOS, 2015.


==> Rebuttal.tex <==
Thanks for the constructive comments. We address all the summarized issues and major issues in individual reviews.

### Summarized Questions
**P1:** Experiment Settings. 

**Reply:** The following table shows the detailed experiment settings.

|Benchmark|Number CN-MN|Index replication factor|Data replication factor|
|---------|------------|------------------------|-----------------------|
|Microbenchmark (Figures 10, 11)|16-2|1|2|
|YCSB (Figures 12, 13, 16)|16-2|1|2|
|YCSB (Figure 14)|16-5|1|2|
|Fault tolerance (Figures 16, 19)|16-5|1~5|1~5|
|Fault tolerance (Figure 17)|16-2|2|2|
|Adaptive Cache & Elasticity (Figures 15, 18)|16-2|1|2|

We set the index replication to 1 for fair comparisons with Clover and pDPM-Direct because the open-source version of Clover only supports a single metadata server, and pDPM-Direct also has no replicated hash index.
We evaluated the performance of FUSES with different numbers of index replicas in Figures 16 and 19. Combining the results of Clover with 1 index replica and 2 data replicas on 5 MNs (Figure 14), FUSES still exhibits higher overall throughput. The following table shows the throughput of FUSES under different numbers of index and data replications.

|Replication (Index-Data)|YCSB-A (Mops)|YCSB-B (Mops)|YCSB-C (Mops)|YCSB-D (Mops)|
|------------------------|-------------|-------------|-------------|-------------|
|FUSES 2-2|6.7|13.4|19.1|16.6|
|FUSES 3-3|4.7|13.3|19.1|16.1|
|Clover 1-2|0.7|3.3|4.8|1.8|


**P2:** How well does FUSES work for larger datasets and for datasets with smaller values?

**Reply:** 
The performance of FUSES does not significantly change for larger datasets because the performance of FUSES depends on the number of RRTs for each kind of operation, which is deterministic, as shown in Figure 9, and agnostic to the dataset size.
Smaller KV pairs make the performance of FUSES better because FUSES is bounded by the network bandwidth and smaller KV pairs consume less NIC bandwidth. 
The following table shows the throughput of FUSES under different sizes of KV pairs with a larger data set (1,000,000 keys).

|KV size|YCBS-A (Mops)|YCSB-B (Mops)|YCSB-C (Mops)|YCSB-D (Mops)|
|-------|-------------|-------------|-------------|-------------|
|1024B|3.3|6.9|9.3|7.7|
|512B|4.0|8.9|13.4|10.8|
|256B|4.1|10.2|14.5|11.6|


**M1:** What problem does FUSES solve?

**Reply:** FUSES addresses the resource utilization issue of the existing partial/semi- memory-disaggregated KV store (Clover). Clover adopts monolithic metadata servers to manage the hash index and memory space. Due to the monolithic nature of its metadata server, Clover still cannot fully exploit the resource utilization and elasticity benefits of the DM architecture. FUSES explores the design of a fully memory-disaggregated KV store that only relies on the computation power of clients and memory space of MNs to achieve full resource utilization on DM.


**D1:** What are the pros and cons of maintaining separate metadata servers vs. storing metadata with the data? Is a fully memory-disaggregated KVS design the only approach for addressing the problem your target?

**Reply:** Compared with metadata servers, storing metadata together with data has the following pros and cons:
- Pros:
    - No additional resources to manage metadata.
    - Better scalability and elasticity. Specifically, the computation power that manages metadata grows and shrinks on demand with the number of concurrent clients.
- Cons:
    - Have to deal with the complex failures situations on DM, which is exactly the challenge that FUSES aims to address.

We believe that the fully memory-disaggregated KVS design is the *ideal* architecture to make KVS fully enjoy the resource utilization and elasticity benefits of DM. The design of FUSES aims to achieve better performance when the computation power of memory nodes is weak. However, there may have other solutions considering the emerging network devices, *e.g.*, SmartNICs and programmable switches.


**D2:** What are the requirements for FUSES' memory management? What can be handled by the client, and what must be handled by MNs? How well would an MN-only solution perform?

**Reply:** The major requirement for FUSES' memory management is to efficiently allocate memory spaces to hold KV pairs. Both clients and MNs can handle the entire memory management tasks. However, allocating memory purely with client-side computation power requires expensive synchronization to guarantee correctness, as discussed in [Ref. 61]. Meanwhile, the weak computation power of MNs cannot handle the frequent fine-grained allocation requests. 
Hence, FUSES proposes to conduct the fine-grained allocation on clients to avoid overwhelming the computation power on MNs, and the coarse-grained allocation on MNs to avoid the expensive synchronization among clients on memory allocations.

An MN-only solution performs poorly due to the weak computation power of MNs. 
The following supplementary experiment compares the FUSES' memory management with the MN-only solution. The throughput of YCSB-A, YCSB-B, and YCSB-D is affected due to the poor computation power on MNs. The throughput of the YCSB-C is not affected due to its read-only nature. We can include the results in the paper for better understanding.

|Approach|YCSB-A (Mops)|YCSB-B (Mops)|YCSB-C (Mops)|YCSB-D (Mops)|
|--------|-------------|-------------|-------------|-------------|
|FUSES's memory management|3.3|6.7|8.8|8.9|
|MN-Only Memory Management|0.3|5.7|8.8|5.5|


**D3:** Please clarify how the proposed 2-level memory allocation/free is used in the context of read and write operations. How does FUSES reclaim the memory space of old KV pairs?

**Reply:** The memory allocation is used for allocating memory spaces for KV pairs. As described in Section 4.1, for *inserts* and *updates*, memory allocation happens before the modification of the hash index. For *updates* and *deletes* operations, the reclamation of old KV pairs happens after the modification of the hash index.

FUSES let clients reclaim their allocated memory blocks, as mentioned in Section 4.3. Clients first check the free bit maps of their allocated memory blocks and reclaim the block by detaching it from the embedded operation log, which is a doubly linked list. In our implementation, garbage collection happens when clients cannot allocate memory from MNs. Due to the deferred reclamation, the concurrency issue of *reads* and memory reclamation mentioned in Review E is rare. To avoid the rare case, FUSES adopts a similar approach in RACE hashing [Ref. 74]. Clients can still access the memory block pointed by the stale pointers. The correctness is guaranteed by checking the stored key and the CRC of the KV pair. We can clarify the implementation in our paper. 


### Other Questions
**D4:** How does FUSES compare with Dinomo? (Review B)

**Reply:** FUSES is different from Dinomo in the following two aspects.
- In Dinomo, KV operations involve three entities, i.e., client, KVS node (KN), and DM. For a KV operation, a client first sends the operation request to a KN. The KN accesses the metadata and KV data in DM and then replies the client. In contrast, KV operations in FUSES only involve two entities, i.e., client and DM. Clients directly access the metadata and KV data in DM without involving the KN, reducing one network RTT.
- Dinomo assumes the memory pool is reliable and fault-tolerant. Consequently, its design does not consider the MN failures. In contrast, FUSES addresses the challenges of reliability and fault tolerance via SNAPSHOT replication.


**P3:** Is the search latency of FUSES without this optimization (adaptive cache) worse than that of Clover? (Review E)

**Reply:**
Theoretically, the *searches* of FUSES have the same number of RTTs compared with Clover without the adaptive cache optimization. The adaptive cache addresses the issue of wasted bandwidths on cache invalidations, as introduced in Section 4.5.1. The operation latency is not affected.


**M2:** How many of your design decisions were in reaction to Clover's architecture vs. choices that you would have proactively made if you were designing FUSES from scratch? (Review B)

**Reply:** All our design choices are made to construct an *ideal* memory-disaggregated KV store on DM that can fully utilize the resource utilization and elasticity benefits of DM.


**D5:** How are the primary and backup replica locations chosen? Are they coordinated? (Review B)

**Reply:** We rely on consistent hashing to choose primary and backup replica locations similar to FaRM [Ref. 19], as discussed in Section 4.3.
No coordination is required when selecting the primary and backup replicas.


**D6:** How do you ensure that the master is fault tolerant? (Review B)

**Reply:** In our paper, we assume the master is fault-tolerant, which is a common assumption in the literature [Ref. 37, 60, 63].
Practically, a fault-tolerant master can be achieved by replicating the master with state-machine replication.


**P5:** Why Clover seems to have lower latency in *searches*? (Review C)

**Reply:** Theoretically, Clover and FUSES have the same number of RTTs on *searches*. The implementation of FUSES concurrently reads KV pairs according to the address in the local cache and two hash buckets according to RACE hashing [Ref. 74], while Clover only reads the KV pair. The minimum latency of FUSES is slightly higher than that of Clover due to the more data read in a single RTT.

**P6:** Discussion of Resource Utilization (Review D)

**Reply:** We have discussed the resource consumption of Clover and FUSES in Section 6.2 and Section 6.3. FUSES achieves better overall throughput even though Clover consumes an additional metadata server.


**D7:** How would the presence of additional DM computational capabilities impact FUSES' design? (Review B)

**Reply:** With additional computation capabilities in SmartNICs, the memory management of FUSES may be able to be conducted on the SmartNICs of MNs. However, the cost of a SmartNIC is much higher than a normal NIC [Ref. 61].


**D8:** How does the FUSES architecture generalize beyond a key-value store to a broader set of applications? (Review B)

**Reply:** In general, other applications can also adopt the fully-disaggregated architecture to have better elasticity and resource utilization. For techniques proposed by FUSES, the two-level memory management and the embedded operation log of FUSES are application-agnostic and hence can be applied to other applications. The SNAPSHOT replication is designed for lock-free hashing indexes. For other types of indexes, new replication protocols need to be proposed.

**Terms** (Review B)
- Partially disaggregated: We can change the term "partially disaggregated" to "semi-disaggregated" to avoid confusion.
- The FUSES-NC refers to the approach without a local cache. The effectiveness of the adaptive cache is evaluated in Figure 15.

==> Sections/trash/05-exe-rec.tex <==
\section{Execution and Recovery}\label{sec:execution}
\noindent
Combining all the above components together, this section introduces how \kv executes KV operations and conducts failure recovery.

\subsection{Operation Execution}
\noindent
Figure~\ref{fig:kv-ops} shows the procedures for executing different KV operations.
Each operation consists of multiple phases with multiple network requests.
For each phase, \kv first leverages PCIe doorbell batching~\cite{designGuideline} to minimize the overhead of transmitting network requests from user processes to RNICs.
\kv then adopts RDMA selective signaling~\cite{designGuideline} to reduce the overhead of polling RDMA completion queues.

For \texttt{INSERT} operations, the KV pair is first written to MNs and then the hash index is modified to point to the address holding the KV pair.
For \texttt{SEARCH} operations, a client simply reads the address stored in the primary slot and then read KV pair from the address.
For \texttt{DELETE} and \texttt{UPDATE} operations, a clients first confirms the slot a KV pair is stored by reading the KV pair. 
The new KV data is written concurrently with doorbell batching.
Then the corresponding hash slot is modified according to \rep replication protocol.
For operations that involve index modification, the log entry is committed before the primary slot is modified.
With this procedure, for \texttt{INSERT}, \texttt{DELETE}, and \texttt{UPDATE} operations, four RTTs are required in general cases.
For \texttt{SEARCH} operations, at most two RTTs are required and in the best case only one RTT is required due to the index caching.

\subsection{Recovery}
Similar to membership-based replication protocols~\cite{hermes,cr,craq}, \kv relies on a fault-tolerant master with a lease-based membership services to tolerate failures.
In this subsection, we first introduce our failure model and then discuss how failures are handled by \kv.
The detailed correctness demonstration can be found in Appendix~\ref{X}.

\subsubsection{Failure Model}
\noindent
We consider a partially synchronous system where processes are equipped with loosely synchronized clocks~\cite{}.
Crash-stop failure can occur, {\em i.e.}, compute node and memory node can fail by crashing and their operation is non-Byzantine.
We consider realistic RDMA network situations in our failure model.
Each client and MN is associated with an RDMA network interface card (RNIC) in our failure model, implying that link failures are equivalent to node crashes~\cite{}.
Guaranteed by RDMA protocol, single-client RDMA operations follows the FIFO order~\cite{ukharon}.
However, there is no guarantee of operation execution orders on MNs.

Under this failure model, \kv guarantees linearizable \texttt{read}s and \texttt{write}s, {\em i.e.}, every operation is atomically committed in a time between its invocation and completion~\cite{lin}.
All the objects of \kv are durable and available under arbitrary number of client crashes and at most $r - 1$ MN crashes, where $r$ is the replication factor.

\subsubsection{Memory Node Failures}
MN failures lead to failed accesses to KV pairs and hash slots.
For the accesses to KV pairs, clients access the backup replicas according to the consistent hashing.

The complication comes from accessing hash index slots.
For \texttt{SEARCH} operations, a failed MN leads to failed primary and backup slots.
On backup slot failures \texttt{SEARCH} operations can execute normally.
On primary slot failures \texttt{SEARCH} operations return the value backup slots if all values in the backup slots are the same.
Otherwise, clients send RPCs to the master and rely on the master to handle the failure and return a correct value. 
For \texttt{INSERT}, \texttt{UPDATE}, and \texttt{DELETE} operations.
All clients, except for the decided last writers send RPCs to the master and rely on the master to return the modified value.
The decided last writers can continue modifying the slots and can modify all alive slots to the same value.

On receiving RPC requests or detecting MN failures, the master first notifies and blocks clients from further issuing KV modification requests to the failed slots.
Then the master randomly select a value in an alive backup slot and modify all alive slots to that value.
Then the master commits the operation log by issuing RDMA \texttt{WRITE} to the commit field of the log header.
After that, the master replies all RPCs with the decided value and choose new primary and backup slots in a new membership view.
On receiving the RPC replies, clients retry their write operation if the return value equals their $v_{old}$, and thus guarantees the correctness.
During the whole process, only accesses to the failed slot is affected and the blocking time can be short thanks to the microsecond-scale membership service~\cite{ukharon}.

\subsubsection{Client Failure}
\noindent
\kv can recover an arbitrary number of client failures.
When a client crashes, the master starts a recovery process or a new client to recover the crashed operation according to the operation log.
The recovery process consists of two steps, {\em i.e.}, 1) memory re-management and 2) operation recovery.
Memory re-management constructs the volatile memory management information of the crashed client, {\em i.e.}, free lists maintained locally on clients.
The recovery process first asks for MNs to get all memory chunks allocated for the crashed client.
Then the per-size-class operation log is traversed to find all the used memory blocks and the crashed operation of the client.
The crashed operation log entry can be identified as the log with incomplete commit pointer and a set used bit.

The operation recovery then repairs the partially modified hash index.
The first step is to identify the crash point of the operation.
Figure~\ref{fig:kv-ops} shows the possible crash points and their corresponding reactions.
Crash points before committing the log (c0 in Figure~\ref{fig:kv-ops} can be distinguished by checking if the ``commit'' field is empty.
The operation that crashes before committing (c0) are retried during recovery.
Crash points after committing the log (c1 or c2) are distinguished by checking the contents in the index slots.
If the content in the primary slot equals to the content in the ``commit'' field, then the operation crashed at c1. 
The recover process modifies the primary slot and finishes the recovery.
Otherwise, the operation crashed at c2 and no recovery is required because the operation is completed.

Under client failures, other clients can read KV pairs.
The index modifications are only blocked when they target the partially-modified KV pairs.
Since the metadata is stored on MNs, an arbitrary number of client crashes can be recovered.

\subsubsection{Mixed Failure}
\noindent
In situations where clients and MNs crash together, we recover the failures separately.
We first let the master recover all MN failures and then start the recovery processes for failed clients.
Operations can proceed because the master acts as the last writer for all blocked operations.
Clients will also not redo committed operations because the master commits the operation logs on clients' behalf.

==> revision-plan.tex <==
Dear Dr. Kimberly Keeton,

Thanks for shepherding our paper #131 “FUSES: A Fully Memory-Disaggregated Key-Value Store”. Based on the reviewers ‘comments, we drew up a revision plan as shown in the following. Please let us know if you have new comments or suggestions. We plan to send you the revised version before Jan. 9th. 

Comment 1: Please provide more details about your experimental setup.
Revision: To avoid confusion, we will make the experimental setup clearer in Section 6 as we presented in the rebuttal.

Comment 2: The YCSB evaluation data set is quite small. How does FUSES work for larger datasets and for datasets with smaller values?
Revision: We will describe our supplementary results of FUSES with larger datasets and small key-value sizes in the paper as we presented in the rebuttal to address this issue.

Comment 3: What problem does FUSES solve?
Revision: We will describe the problem clearly in the introduction (Section 1) and background (Section 2).

Comment 4: What are the pros and cons of maintaining separate metadata server VS. storing metadata with the data? Is a fully memory-disaggregated KVS design the only approach to address the problem your target?
Revision: We will discuss the pros and cons in Section 7.

Comment 5: What are the requirements for FUSES’ memory management, and what can be handled by the client vs. what can be handled by the memory node? How well would an MN-only solution perform?
Revision: We will specify the requirements of FUSES’ memory management in Section 4.3, as we explained in the rebuttal. We will also add the results of FUSES with MN-only memory management in Section 6.

Comment 6: Please clarify how the proposed 2-level memory allocation/free is used in the context of read and write operations.
Revision: We will present more details of 2-level memory management in Section 4.3 to avoid confusion.

Comment 7: How does FUSES compare with Dinomo? 
Revision: We will discuss the differences between FUSES and Dinomo in Section 7.

Comment 8: Is the search latency of FUSES without adaptive cache worse than that of Clover?
Revision: We will explain the reason in Section 6, as we explained in the rebuttal.

Comment 9: How are primary and backup replica locations chosen? Are they coordinated?
Revision: We will clarify this in Section 4.3, i.e., we use consistent hashing to select primary and backup replicas.

Comment 10: How would additional DM computational capabilities impact FUSES’ design? 
Revision: We will discuss this in Section 7.

Comment 11: The term “partially disaggregated” may cause confusion because it has already been defined as an architecture where compute nodes have a small amount of local memory.
Revision: We will change the term to “semi-memory-disaggregated” to avoid confusion.

Comment 12: Readers may not be familiar with the RACE hashing paper.
Revision: We will briefly introduce RACE hashing in Section 4.1 for self-containment.

Comment 13: The two-level memory management is reminiscent of what HP did in The Machine.
Revision: We will discuss the similarities and differences in Section 7.

Comment 14: You describe FUSES-NC as the version of FUSES without the adaptive index cache. Does that mean it doesn’t have the adaptive cache or no local cache at all?
Revision: We will clarify that FUSES-NC is the version without a local cache in Section 6.

Comment 15: The name “FUSES” is strange to have the system's name look like a plural English word.
Revision: We plan to change the acronym afterward.

Besides, we will carefully proofread the final version of the paper.


Best,
Jiacheng.

